Logical Abstractions for Noisy Variational Quantum Algorithm Simulation

Due to the unreliability and limited capacity of existing quantum computer prototypes, quantum circuit simulation continues to be a vital tool for validating next generation quantum computers and for studying variational quantum algorithms, which are among the leading candidates for useful quantum computation. Existing quantum circuit simulators do not address the common traits of variational algorithms, namely: 1) their ability to work with noisy qubits and operations, 2) their repeated execution of the same circuits but with different parameters, and 3) the fact that they sample from circuit final wavefunctions to drive a classical optimization routine. We present a quantum circuit simulation toolchain based on logical abstractions targeted for simulating variational algorithms. Our proposed toolchain encodes quantum amplitudes and noise probabilities in a probabilistic graphical model, and it compiles the circuits to logical formulas that support efficient repeated simulation of and sampling from quantum circuits for different parameters. Compared to state-of-the-art state vector and density matrix quantum circuit simulators, our simulation approach offers greater performance when sampling from noisy circuits with at least eight to 20 qubits and with around 12 operations on each qubit, making the approach ideal for simulating near-term variational quantum algorithms. And for simulating noise-free shallow quantum circuits with 32 qubits, our simulation approach offers a $66\times$ reduction in sampling cost versus quantum circuit simulation techniques based on tensor network contraction.

==> 41_evaluation.tex <==
% Performing quantum circuit simulation using knowledge compilation offers three capabilities:
% \begin{enumerate}
% \item Reduction of the simulation problem complexity;
% \item Efficient repeated simulation of quantum circuits with the same topology but different parameters;
% \item Efficient repeated simulation of the same quantum circuits with different measurement outcomes.
% \end{enumerate}
% We evaluate each of these benefits using different quantum algorithm workloads in this section.
% These features improve our ability to simulate quantum circuits,
% which may have transformational impact on our ability to develop quantum algorithms.

\subsection{Simulation for Different Measurement Results}

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{figures/unstructured_workloads.pdf}
\caption{Metrics for simulating random circuit sampling using knowledge compilation.
}
\label{fig:unstructured_workloads}
\end{figure}

Finally, we evaluate our toolchain's ability to more efficiently perform repeated simulations with different assignments of states to the outcomes.
This type of repeated inference is useful for a class of quantum simulations in the area of quantum supremacy.
Quantum supremacy is a milestone in quantum computing research where a quantum computer is able to solve a problem faster than any classical approach~\cite{Harrow,Terhal}.
% Researchers have been pushing the limits of quantum program simulation, in order to probe the boundary between classical and quantum computing~\cite{}.

Specifically, we simulate the quantum random circuits sampling workload~\cite{boixo2018supremacy},
a class of circuits proposed as benchmarks for whether a quantum computer truly exceeds the capability of classical computers~\cite{Harrow,pednault2017breaking,Terhal}.
In this class of simulations, we need to sample the output probability distribution of a quantum computer,
which in this case entails repeated inferences on the same Bayesian network but with different sets of evidence.
Prior work in simulating RCS workloads has hinted that reusing part of the simulation across samples is key to scaling to larger simulations~\cite{boixo2017simulation}.
This work is the first demonstration of doing that using classical knowledge compilation techniques.

In Figure~\ref{fig:unstructured_workloads}, the plots are the arithmetic circuit file size, AC compilation time, and simulation time for each measurement outcome, plotted against the RCS circuit depth.
The simulation time for each outcome (rightmost plot) can be directly compared against results by Boixo et al.~\cite{boixo2017simulation}, which is also a workstation-scale simulation of the same workload.
For RCS simulations of depth 17-29, our simulation time per measurement outcome is faster by up to $20\times$ for smaller simulation sizes.
The faster simulation time for these problem sizes is due to precompilation of the circuit structure through knowledge compilation.

The knowledge compilation approach faces scalability challenges due to having to work with large arithmetic circuits for large problem sizes, which is expected due the intractability of quantum simulation.
For problem sizes beyond depth 29, the qubit states become increasingly entangled resulting in less independence structure.
With less independence structure, the exponential growth of the AC file size (leftmost plot) removes the advantage of knowledge compilation.

% \paragraph{First generation (cZ gate) benchmark}
  % \subsection{cZ benchmarks}
  % ${H, T, C(Z), X^.5, Y^.5}$
  % ${x^.5, y^.5, T}$
  % (T is the weird one out)
  % $x^1/2 = sqrt(x) = HSH$
  % $Y = S X Sdg = SXSSS$
  % $y^1/2 = sqrt(y) = SHSHSSS$
% \paragraph{Second generation (iSWAP gate) benchmark}
  % First report of simulation performance of new generation of quantum benchmarks
  % iSWAP diagonalizable version (symmetric) vs. Non diagonalizable (asymmetric) version
  % PSWAP(theta) = [[1,0,0,0],[0,0,e^(jtheta),0],[0,e^(jtheta),0,0],[0,0,0,1]]
  % SWAP = PSWAP(0) = [[1,0,0,0],[0,0,1,0],[0,1,0,0],[0,0,0,1]]
  % iSWAP = PSWAP(pi/2) = [[1,0,0,0],[0,0,j,0],[0,j,0,0],[0,0,0,1]]
  % Decomposition to cx, s, cx, cx helps

% With our toolchain, we are able to compile the arithmetic circuit once up front,
% and perform repeated simulation of the circuit with different evidence.
% With sufficient samples, our simulation results converge to the Porter-Thomas distribution depicted in Figure~\ref{fig:porter-thomas},
% which validates that the simulation results are correct.
% The reason that random benchmarks start to scale not as well is because random matrices do not have as much independence

% Randomly choose a txt file
% Randomly pick which bit to flip
% Statistical consensus across different draws
% Summarize outputs
% evaluationDuration mean and variance for a given instance
% Statistical consensus across different txt files
% mean and variance across instances

% Competition against various other prior work on quantum supremacy simulations
% The competition
% 6x6 20 - 40 depth
% 7x7 20 - 40 depth
% 7x7 qubits depth 25
% would need a petabyte of storage
% 7x7 qubits depth 27

% Harrow: "Developing good classical simulations (or even attempting to and failing) would also help clarify the quantum/classical boundary."
% This will be interesting to this audience; they like new benchmarks.
